Leveraging QA Datasets to Improve Generative Data Augmentation

The ability of generative language models (GLMs) to generate text has improved considerably in the last few years, enabling their use for generative data augmentation. In this work, we propose CONDA, an approach to further improve GLMs' ability to generate synthetic data by reformulating data generation as context generation for a given question-answer (QA) pair and leveraging QA datasets for training context generators. Then, we cast downstream tasks into the same question answering format and adapt the fine-tuned context generators to the target task domain. Finally, we use the fine-tuned GLM to generate relevant contexts, which are in turn used as synthetic training data for their corresponding tasks. We perform extensive experiments on multiple classification datasets and demonstrate substantial improvements in performance for both few- and zero-shot settings. Our analysis reveals that QA datasets that require high-level reasoning abilities (e.g., abstractive and common-sense QA datasets) tend to give the best boost in performance in both few-shot and zero-shot settings.

==> files/3-prelims.tex <==
% \section{Problem Formulation}

% For a given task $\mathcal{T}$, the input in a few-shot setting contains a very small labeled dataset $\mathcal{L}_\mathcal{T} = \{(\mathcal{D}_1, l_1), (\mathcal{D}_2, l_2), \ldots, (\mathcal{D}_{|\mathcal{L}_\mathcal{T}|}, l_{|\mathcal{L}_\mathcal{T}|})$\} 
% % (2) large corpus of unlabeled documents $\mathcal{U}_\mathcal{T} = \{\mathcal{D}_1, \mathcal{D}_2, \ldots, \mathcal{D}_{|\mathcal{U}_\mathcal{T}|}$\}, 
% and $m$ target classes $\mathcal{C}$ = \{$\mathcal{C}_1, \mathcal{C}_2, \ldots, \mathcal{C}_m$\}.
% % The unlabeled data set $\mathcal{U}_\mathcal{T}$ can be artificially created by removing the ground truth labels of labeled documents.
% Our method requires users to provide a question per dataset that is representative of the task to be solved.
% % \todo{write about question representing task}
% Our aim is to build a model for the task $\mathcal{T}$ that assigns a label $\mathcal{C}_j \in \mathcal{C}$ to each document $\mathcal{D}$. 
% % \timo{It said $D_i$ here, I replaced it with a more general $D$ because we do not want to only assign labels to the training data, but to arbitrary documents $D$.}

% % \newpoint{Explain the problem, input output}


==> files/4-method.tex <==
% \section{Intermediate Training on QA Datasets}
% % \timo{Not every QA dataset has this format, so I slightly reworded this}
% We consider question-answering datasets $Q$ containing triplets $(q,a,c)$ of a question $q$, the corresponding answer $a$, and a context $c$ required to derive the correct answer.
% Question-answering datasets can roughly be divided into \emph{extractive}~\cite{rajpurkar-etal-2016-squad, trischler-etal-2017-newsqa, joshi-etal-2017-triviaqa, reddy2019coqa} and \emph{abstractive} datasets~\cite{kocisky-etal-2018-narrativeqa, huang-etal-2019-cosmos, xiong2019tweetqa, sap-etal-2019-social}.
% % \timo{Would be good to have a few citations here for extractive and abstractive datasets, respectively.}
% For extractive QA datasets, the answer can be found as a contiguous span in the context, whereas in abstractive QA datasets, the answer needs to be generated in natural language without being able to rely on the vocabulary of the
% question or context.
% % \timo{I removed some text here as I don't really think the information is necessary}
% %All common-sense QA datasets are abstractive in nature.
% %Since we aim to train a context generator, we don't require span information and only consider questions, answers, and contexts for all QA datasets.

% We transform the QA dataset $Q$ into training data $D_{QAC}$ for fine-tuning the GLM.
% To this end, each triplet ($q$, $a$, $c$) is converted into a single text by prepending \textit{``question:''}, \textit{``answer:''} and \textit{``context:''}, respectively, and concatenating $q$, $a$ and $c$ separated by newlines.
% % \timo{ Note that the boxes violate the margin rules, this should be fixed.}
% For example, a preprocessed training document obtained from an extractive QA dataset might look like the following:\\

% \noindent\fbox{%
%     % \parbox[t]{7.5cm}{
%     % \parbox{\columnwidth}{
%     \parbox{0.95\linewidth}{
%         \textcolor{red}{\texttt{question}}: when did battle of plassey happen?\\
%         \textcolor{red}{\texttt{answer}}: 23 june 1757 \\
%         \textcolor{red}{\texttt{context}}: the battle of plassey was a decisive victory of the british east india company over the nawab of bengal and his french allies on 23 june 1757.
%     }
% }
% \\

% We fine-tune a pretrained GLM $G$ on $D_{QAC}$ to obtain a \emph{general context generator} $G_Q$ using a language modeling objective to maximize the log-likelihood of the ($q$, $a$, $c$) triplet. 
% % \timo{I don't think the mathematical part here is necessary as the NLL formulation should be known to the reader. Also, I don't think the equation is correct. Why would $(P(q_i, a_i, c_i; \Theta))$ be the same as $P(c_i|q_i, a_i; \Theta)$?}
% %Mathematically, for a given question $q_i$, answer $a_i$, and context $c_i$, we learn parameters $\Theta$ by maximizing $\mathcal{L}$ where:
% %\begin{align*}
% %    \mathcal{L} =  \sum_ilog(P(q_i, a_i, c_i; \Theta)) \\
% %    = \sum_ilogP(c_i|q_i, a_i; \Theta)
% %\end{align*}
% %One can view our formulation as asking the question $q_i$ and answer $a_i$ to play the role of prompt and the context
% %$c_i$ to be the continuation, thus facilitating conditional context generation.
% We call this step QAC fine-tuning.

% % This language modeling loss facilitates conditional generation of context given question and answer, which we discuss in detail in next section.
% % In our experiments, we use GPT2-medium~\cite{Radford2019LanguageMA} as $G$.

% \section{Domain Adaptation and Synthetic Training Data Generation}
% % \newpoint{Context generator and using questions and answers}

% We adopt $G_Q$ to the target domain by fine-tuning it further on available few-shot data.
% To preserve its context generating ability, we perform QAC fine-tuning instead of regular language model fine-tuning.
% This is enabled by transforming the few-shot supervision into our question-answer-context format.
% First, we manually design one question per dataset that is representative of the task and the dataset. 
% Furthermore, following ~\citet{schick-schutze-2021-exploiting}, we define a verbalizer as a mapping $v$: $\mathcal{C} \rightarrow \mathcal{V}$ that maps each label in $\mathcal{C}$ to a word from $G_Q$’s vocabulary $\mathcal{V}$.
% Finally, for every document $\mathcal{D}_i$ and its respective label $l_i$ in our few-shot data, we consider the verbalizer mapping of the label, $v(l_i)$, as answer and the text $\mathcal{D}_i$ as context.
% For example, a \textit{negative} review \textit{``I hate this movie''} from the IMDb dataset \citep{maas-EtAl:2011:ACL-HLT2011} is transformed as follows:\\

% \noindent\fbox{%
%     % \parbox[t]{7.5cm}{
%     % \parbox{\columnwidth}{
%     \parbox{0.95\linewidth}{
%         \textcolor{red}{\texttt{question}}: is the movie good or bad?\\
%         \textcolor{red}{\texttt{answer}}: bad \\
%         \textcolor{red}{\texttt{context}}: i hate this movie.
%     }
% }
% \\

% We fine-tune $G_Q$ on the converted few-shot data to obtain a target task context generator $G_\mathcal{T}$. 


% \paragraph{Synthetic Training Data Generation} Recall that our method requires a question $q$ for every dataset that is representative of the task to be solved.
% To obtain synthetic training data, for every distinct label $\mathcal{C}_j$, we create a question-answer prompt with $q$ as question, $v(\mathcal{C}_j)$ as answer and let $G_\mathcal{T}$ generate the context $c_{gen}$.
% % \timo{I'm pretty sure that the following equation is wrong - obtaining the argmax would be intractable, which is why we would practically use some approximation like greedy decoding or beam search. But then again, we don't do that either as we sample from our distribution. I would just remove this equation alltogether.}
% %Specifically, given question $q$ and answer $v(\mathcal{C}_j)$, we conditionally generate $c_{gen}$ using $P(c_{gen}|q, a)$ probabilities from $G_\mathcal{T}$:
% %\begin{align*}
% %    c_{gen} = \arg\max_c P(c | q, a)
% %\end{align*}
% The generated context $c_{gen}$ and label $\mathcal{C}_j$ are considered as a synthetic training sample. 
% We repeat this process multiple times to generate $n$ samples that we collect in a synthetic training dataset denoted by $\mathcal{D}_{gen}$.

% As a final step, we train the target task model on the combination of $\mathcal{D}_{gen}$ and our original few-shot dataset $\mathcal{L}_\mathcal{T}$.
% We use this trained target-task model for inference. 
